Efficient and Optimal Algorithms for Tree Summarization with Weighted Terminologies

Data summarization that presents a small subset of a dataset to users has been widely applied in numerous applications and systems. Many datasets are coded with hierarchical terminologies, e.g., the international classification of Diseases-9, Medical Subject Heading, and Gene Ontology, to name a few. In this paper, we study the problem of selecting a diverse set of k elements to summarize an input dataset with hierarchical terminologies, and visualize the summary in an ontology structure. We propose an efficient greedy algorithm to solve the problem with (1-1/e) = 62% -approximation guarantee. Although this greedy solution achieves quality-guaranteed answers approximately but it is still not optimal. To tackle the problem optimally, we further develop a dynamic programming algorithm to obtain optimal answers for graph visualization of log-data using ontology terminologies called OVDO . The complexity and correctness of OVDO are theoretically analyzed. In addition, we propose a useful optimization technique of tree reduction to remove useless nodes with zero weights and shrink the tree into a smaller one, which ensures the efficiency acceleration of OVDO in many real-world applications. Extensive experimental results on real-world datasets show the effectiveness and efficiency of our proposed approximate and exact algorithms for tree data summarization.

==> exp.tex <==
\section{Experiments}\label{sec.exp}

%In this section, we conduct experiments on real-world datasets to evaluate the efficiency and effectiveness of our algorithm. 
%In this section, we test our algorithms in experiments.

In this section, we conducted extensive experiments to evaluate the performance of our proposed methods. All algorithms are implemented in C++. \TKDE{The source codes are publicly avaliable.\footnote{\url{https://github.com/csxlzhu/TKDE_OVDO}} Experiments are conducted on a Linux Server with Intel Xeon X5650 (2.67 GHz) and 32GB main memory.}

\begin{table}[t]
%\vspace{-0.2cm}
\centering
%\vspace{-0.3cm}
\caption{The statistics of tree datasets.}\label{table:data}
\vspace{-0.3cm}
\scalebox{1.0}{
\begin{tabular}{c|c|c|c}
\toprule
Name& $n$& $|\mathcal{I}|$& Height\\
\midrule
\LATT& 4,226& 960& 22\\
\LNUR& 4,226& 771& 22\\
\ANIM& 15,135& 4,350& 11\\
\IMAGE& 73,298& 5,000& 20\\
\YAGO& 493,839& 10,000& 17\\
\bottomrule
\end{tabular}
}
%\vspace{-0.2cm}
%\vspace{-0.5cm}
\vspace{-0.5cm}
\end{table}

\stitle{Datasets. } We use five real-world datasets of hierarchical tree $T$ containing weighted terminologies. First, \LATT and \LNUR are extracted from the Medical Entity Dictionary (MED) \cite{jing2011graphical}. The tree contains 4,226 nodes. In addition, we use two datasets of $\mathcal{I}$, where the dataset \LATT contains the information about how physicians query online knowledge resources, and the other dataset \LNUR contains the query information of nurses. These two datasets contain 960 records and 771 records, respectively. Each record consists of a MED term with a frequency count of its occurrence in the log file. 
The third dataset, \ANIM, is extracted from the "Anime" catalog in Wikipedia \cite{ANIM}. The \ANIM tree contains 
15,135 vertices. Each vertex represents the animation websites or superior categories.
%The 15,135 vertices represent the animation websites or superior categories. 
The weight of a vertex is the number of page-views on this vertex catalog within one month. 
The fourth dataset, \IMAGE, is extracted from the Image-net \cite{imagenet}. The \IMAGE tree contains 
73,298 vertices.
Each \emph{synset} tag represents a vertex, whose id is given in the \emph{wnid} attribute of the tag. 
We choose 5,000 random catalogs containing images as the set $I$. The frequency of each catalog is the number of images in the catalog. Last, the fifth dataset, \YAGO, is extracted from the ontology structure yagoTaxonomy in multilingual Wikipedias~\cite{yago, mahdisoltani2013yago3}. The \YAGO tree contains 493,839 taxonomy vertices. An edge represents that the child vertex is a ``subClassOf'' the parent vertex. The frequency of each taxonomy vertex is the number of objects from yagoTypes belong to this taxonomy.\revision{}
%Each record consists of a MED term for the concept of interest and a frequency count of its occurrence in the original infobutton log file. 

\begin{figure*}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure[\LATT]{
\label{fig.exp1_1_1}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_LATT_CD.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\LNUR]{
\label{fig.exp1_1_2}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_LNUR_CD.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\ANIM]{
\label{fig.exp1_1_3}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_ANIM_CD.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\IMAGE]{
\label{fig.exp1_1_4}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_IMAGE_CD.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\YAGO]{
\label{fig.exp1_1_5}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_YAGO_CD.eps} }%\hskip -0.15in
}
\vspace{-0.3cm}
\caption{Closeness distance of different models on all datasets.}% Here, $k=25$.}
\label{fig.exp1_1}
\vspace{-0.4cm}
\end{figure*}

\begin{figure*}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure[\LATT]{
\label{fig.exp1_2_1}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_LATT_ALD.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\LNUR]{
\label{fig.exp1_2_2}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_LNUR_ALD.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\ANIM]{
\label{fig.exp1_2_3}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_ANIM_ALD.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\IMAGE]{
\label{fig.exp1_2_4}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_IMAGE_ALD.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\YAGO]{
\label{fig.exp1_2_4}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_YAGO_ALD.eps} }%\hskip -0.15in
}
\vspace{-0.3cm}
\caption{Average level difference of different models on all datasets.}% Here, $k=25$.}
\label{fig.exp1_2}
\vspace{-0.4cm}
\end{figure*}

\begin{figure*}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure[\LATT]{
\label{fig.exp1_3_1}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_LATT_WC.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\LNUR]{
\label{fig.exp1_3_2}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_LNUR_WC.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\ANIM]{
\label{fig.exp1_3_3}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_ANIM_WC.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\IMAGE]{
\label{fig.exp1_3_4}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_IMAGE_WC.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\YAGO]{
\label{fig.exp1_3_5}
\includegraphics[width=0.205\linewidth]{./Figure/EXP1_YAGO_WC.eps} }%\hskip -0.15in
}
\vspace{-0.3cm}
\caption{Weighted coverage of different models on all datasets.}% Here, $k=25$.}
\label{fig.exp1_3}
\vspace{-0.4cm}
\end{figure*}

\stitle{Compared methods. }
To evaluate %the quality of %our algorithm \greedy, we evaluate and compare three algorithms 
%our model 
the effectiveness of our modeling problem \kVDOmodel, we evaluate and compare four competitive approaches 
-- \textbf{\FEQ}, \textbf{\AGG}, \textbf{\CAGG}~\cite{jing2011graphical}, and \textbf{\TS}~\cite{kimsummarizing}. 

\squishlisttight
\item  \textbf{\FEQ}: is a baseline approach, which selects $k$ nodes with the highest frequencies~\cite{jing2011graphical}.  

\item \textbf{\AGG}:  picks a set of $k$ nodes with the highest aggregate frequencies, where the aggregate frequency of a node $x$ is defined as $AF(v)=\sum_{y\in \dec(x)} \feq(y)$. 

\item  \textbf{\CAGG}: is a variant method of \textbf{\AGG} using another metric of contribution ratio. For a node $x$, the contribution ratio of $x$ is defined by $R(v)=\frac{AF(x)}{AF(y)}$ where $y$ is the parent of $x$. 
%The contribution ratio of root $r$ is $R(r)=1$. 
 Given a ratio threshold $\theta$, \CAGG selects the $k$ nodes that have the highest aggregate frequencies and the contribution ratio no less than $\theta$. We set $\theta=0.4$ by following \cite{jing2011graphical}. 
\item  \textbf{\TS}: is the state-of-the-art method of \underline{T}ree \underline{S}ummaries, which creates a concise summary of similar weights in hierarchical multidimensional data~\cite{kimsummarizing}. To make a comparison, we use the 1-dimensional hierarchical data and a variant setting to select exact $k$ summary vertices as the answer. 
%and assign weights to a few selected vertices in the hierarchy. The objective is to control the estimation error between the summary vertices and the selected vertices~\cite{agarwal2007efficient, kimsummarizing}.%\revision{}
\end{list}

Furthermore, we evaluate the effectiveness and efficiency of our algorithms \greedy (Algorithm~\ref{algo:greedy}) and \DP (Algorithm~\ref{algo:dp}), which respectively solve \kVDO approximately and optimally. We compare them with \Baseline greedy method and \brute. \Baseline greedy method gets the same solution as \greedy, and \brute achieves the same answer as \DP. Furthermore, \Baseline takes $O(n^2)$ time to compute $\triangle_{g}(x|S)$. Thus, the total time complexity of \Baseline is $O(n^3k)$. On the other hand, \brute takes the exponential time w.r.t. the size of tree $|T|$ and parameter $k$. 


%For all methods, we set the parameter $k=25$ by default.
%\textbf{\bulk} is an improved greedy algorithm in Algorithm \ref{algo:bulk}, which removes a set of nodes with size $\frac{\epsilon}{1+\epsilon} |V(G_i)|$ from graph $G_i$ in each iteration. We empirically set $\epsilon = 0.03$.  \textbf{\LATC} is the bottom-up local exploration approach in Algorithm \ref{algo:local}. For all methods, we set the parameter $k=4$ and $d=4$ by default. For \LATC, we empirically set the parameter $\eta = 1000$ and $\gamma = 0.2$, where $\eta=1000$ is selected in order to achieve stable quality and efficiency by testing $\eta$ in the range $[100, 2000]$, and $\gamma = 0.2$ is selected to balance the cohesive structure and homogeneous  attributes for communities explored.

\stitle{Evaluation metrics.}
To evaluate the quality of summary result $S$ found by all models, we use three metrics, i.e., the closeness distance $\CD(\mathcal{I}, S)$~\cite{huang2017ontology}, the average level difference $\ALD(\mathcal{I}, S)$~\cite{zhu2020top}, and also the weighted coverage $\WC(\mathcal{I}, S)$~\cite{zhu2020top}. 

\squishlisttight
\item[1.] The closeness distance $\CD(\mathcal{I}, S)$ is defined as the sum of weighted distance between $S$ to $\mathcal{I}$, denoted by 
$$\CD(\mathcal{I}, S) = \sum_{y\in \mathcal{I}} \min_{x\in S} \dist_{T}(x, y) \cdot \feq(y),$$
where $\dist_{T}(x, y)$ is the number of edges connecting $x$ and $y$ in tree $T$. The smaller is $\CD(\mathcal{I}, S)$, the better is the summary quality.
%, indicating a better prediction of future query

\item[2.] The average level difference  $\ALD(\mathcal{I}, S)$ is a distance-based metric proposed in~\cite{zhu2020top}. $\ALD(\mathcal{I}, S)$ is defined as the average level difference between summary vertex and weighted vertex, denoted by 
$$\ALD(\mathcal{I}, S) =\frac{\sum_{y \in \mathcal{I}} \min_{x\in S \cap \anc(y)} (\l(y) - \l(x)) \cdot \feq(y)}{\sum_{y \in \mathcal{I}} \feq(y)}.$$
Note that we consider $\min_{x\in \emptyset} (\l(y) - \l(x)) = \l(y)$. 
The $\ALD(\mathcal{I}, S)$ metric takes into account both the level difference of summary results and the vertex weight. 
%The $\ALD(\mathcal{I}, S)$ metric can measure the diversity and correlation of the selection. 
The smaller is $\ALD(\mathcal{I}, S)$, the better is the summary quality.


\item[3.] The weighted coverage $\WC(\mathcal{I}, S)$  is defined as the total weight of the vertices within summary set $S$ or their children, denoted by 
$$\WC(\mathcal{I}, S)=\sum_{x \in \mathcal{I} \cap C(S)}{\feq(x)},$$
where $C(S)= S \cup \bigcup_{x \in S} \nb^{-}(x)$. 
The $\WC(\mathcal{I}, S)$ metric evaluates the coverage of important vertices with large weights. The larger is $\WC(\mathcal{I}, S)$, the better is the summary quality. 
%Both average level difference and weighted coverage are also adopted in~\cite{zhu2020top}.
%\revision{The weighted coverage can measure the coverage of the selection. The larger is $\WC(\mathcal{I}, S)$, the better is the summary. Both average level difference and weighted coverage are also adopted in~\cite{zhu2020top}.}
\end{list}

% Second, the average level difference and  $\ALD(\mathcal{I}, S)$ is defined as weighted average level difference between representative vertex and represented vertex, denoted by 
% $$\ALD(\mathcal{I}, S) =\frac{\sum_{y \in \mathcal{I}} \min_{x\in S \cap \anc(y)} (\l(y) - \l(x)) \cdot \feq(y)}{\sum_{y \in \mathcal{I}} \feq(y)}.$$
% Note that we consider $\min_{x\in \emptyset} (\l(y) - \l(x)) = \l(y)$. \revision{The average level difference can measure the diversity and correlation of the selection.} The smaller is $\ALD(\mathcal{I}, S)$, the better is the summary.

% Third, the weighted coverage $\WC(\mathcal{I}, S)$ is defined as the total weight of the vertices within summary set $S$ or their children, denoted by 
% $$\WC(\mathcal{I}, S)=\sum_{x \in \mathcal{I} \cap C(S)}{\feq(x)},$$
% where $C(S)= S \cup \bigcup_{x \in S} \nb^{-}(x)$. \revision{The weighted coverage can measure the coverage of the selection. The larger is $\WC(\mathcal{I}, S)$, the better is the summary. Both average level difference and weighted coverage are also adopted in~\cite{zhu2020top}.}

Generally, both $\CD(\mathcal{I}, S)$ and $\ALD(\mathcal{I}, S)$ measures the distance between selection answer $S$ and important vertices $\mathcal{I}$. The smaller is the value, the better is the summary quality. Overall, these three evaluation metrics admit the desiderata metrics of a good summarization in Section~\ref{sec.pre}. 

To evaluate the effectiveness of algorithms, we also use summary score $\g(S)$ to compare the summary results. The larger is $\g(S)$, the better is the solution. Furthermore, to evaluate the efficiency, we report the running time of different summarization algorithms.  The smaller is the running time, the better is the efficiency. Note that we treat the running time as infinite if the algorithm run exceeds 3 hours. 


% \begin{figure}[t]
% %\vskip -0.6cm
% \small
% \centering 
% \mbox{
% %\hskip -0.1in
% \subfigure[physician]{\includegraphics[width=0.5\linewidth]{./Figure/dis-patient.eps}}
% %\hskip -0.1in
% \subfigure[nurses]{\includegraphics[width=0.5\linewidth]{./Figure/dis-nurse.eps}}
% }
% %\vskip -0.2in
% \caption{Quality evaluation on \emph{physician} and \emph{nurses} data}
% %\vskip -0.1in
% \label{fig.quality}
% \end{figure}

\subsection{Effectiveness Evaluation}

\stitle{Exp-1: Quality comparison of different summarization models.} We compare the summarization quality of five different models \kVDOmodel, \FEQ, \AGG, \CAGG, and \TS. 
Figures \ref{fig.exp1_1}, \ref{fig.exp1_2} and \ref{fig.exp1_3} show the results of competitive methods on all real-world datasets, in terms of the closeness distance, the average level difference, and the weighted coverage, respectively. Note that we use \DP algorithm for \kVDOmodel model, which achieves the optimal solution. The size of summary set $k$ varies from $10$ to $90$. All models achieve smaller closeness distance, average level difference and larger weighted coverage with the increased $k$. Note that the closeness distance of \AGG has a sudden drop on
\LATT and \LNUR from $k=10$ to $30$ as shown in Figures~\ref{fig.exp1_1}(a) and~\ref{fig.exp1_1}(b). This is caused by that the key vertices for tree summarization are selected by \AGG when a large summarization answer $k=30$ but not a small answer $k=10$. Correspondingly, the closeness distance of \AGG reduces significantly. On the other hand, our method \kVDOmodel can target these key vertices to obtain small closeness distances even when a small value $k=10$, reflecting a superiority of \kVDOmodel against \AGG. Furthermore, our model \kVDOmodel is a clear winner of all competitors, consistently achieving the smallest closeness distance, the smallest average level difference, and also the largest weighted coverage in Figures \ref{fig.exp1_1}, \ref{fig.exp1_2} and \ref{fig.exp1_3}.  It significantly outperforms the other methods for a smaller $k$, which is a great help to shrink large datasets for tree summarization. %The similar results can be observed in Figure \ref{fig.quality}(b).

\begin{table}[t]
%\vspace{-0.2cm}
\centering
%\vspace{-0.3cm}
\caption{Summary scores of \greedy and \DP, here $k = 25$}\label{table.exp2}
\vspace{-0.3cm}
\scalebox{1.0}{
\begin{tabular}{c|c|c|c|c|c}
\toprule
Datasets& LATT& LNUR& ANIM& IMAGE& YAGO \\
\midrule
\greedy& 4,071& \textbf{5,048} & 18,628& 542,872& 1,492,101\\
\DP& \textbf{4,111} & \textbf{5,048} & \textbf{18,786}& \textbf{546,368}& \textbf{1,495,580}\\
\bottomrule
\end{tabular}
}
%\vspace{-0.2cm}
%\caption{The results of $\g(S)$ on  tree datasets}\label{table.exp2}
%Summary score $\g(S)$ of \GVDO and \DP on  tree datasets}\label{table.exp2}
\vspace{-0.5cm}
\end{table}

\stitle{Exp-2: Summary score comparison of greedy and optimal algorithms.}
We next conduct the effectiveness evaluation of our algorithm \greedy and \DP. Table~\ref{table.exp2} shows the summary scores of \greedy and \DP on five datasets. The exact algorithm \DP consistently outperforms \greedy on all datasets except \LNUR, verifying the effectiveness of our optimal solution against the greedy approach. 

\begin{figure*}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure[Summary score $\g(S)$]{
\label{fig.exp5_1}
\includegraphics[width=0.29\linewidth]{./Figure/EXP5_1.pdf} }%\hskip -0.15in
\hspace{1.0cm}
\subfigure[Running time(Seconds)]{
\label{fig.exp5_2}
\includegraphics[width=0.29\linewidth]{./Figure/EXP5_2.pdf} }%\hskip -0.15in
%\hspace{-0.29cm}
}
\vspace{-0.3cm}
\caption{Evaluation on 200 small synthetic datasets.}% Here, $k=25$.}
\label{fig.exp5}
\vspace{-0.3cm}
\end{figure*}

\stitle{Exp-3: Approximation evaluation on small synthetic datasets.}
In this experiment, we evaluate the approximation of our algorithms w.r.t. the optimal answers. We randomly generate $200$ small-scale trees with $20$ nodes. 
We compare three methods of \greedy, \DP, and \brute. Note that \greedy produces no optimal solution in these cases. \DP and \brute always produce optimal answers.
Figure~\ref{fig.exp5_1} shows the summary score of three methods on $200$ cases. \DP gets the same solution of \brute, which verify the correctness of \DP.
As we can see that \DP wins the \greedy in all cases and \greedy achieves the average 95\%-approximation of optimal solutions. 
%Obviously, in most cases, EXT-greedy reaches the optimal solution. After statistics, in nearly 75\% cases, EXT-greedy is the same as brute force and only in 20\% cases, the EXT-greedy is still same as greedy+. Moreover, the EXT-greedy is average 99\%-approximation of optimal solution, however, greedy+ is only 95\%. 
Figure~\ref{fig.exp5_2} shows the running time of three methods on all cases. \greedy and \DP run much faster than \brute, and \greedy is the winner. 

% \begin{figure}[t]
% %\vskip -0.1cm
% \small
% \centering 
% %\mbox{\hskip -0.1in
% % \subfigure[physician]{\includegraphics[width=0.5\linewidth]{./Figure/dis-patient.eps}}\hskip -0.1in
% %\subfigure[nurses]{\includegraphics[width=0.5\linewidth]{./Figure/dis-nurse.eps}}
% %}
% \includegraphics[width=0.5\linewidth]{./Figure/scability-v.eps}
% %\vskip -0.2in
% \caption{Scalability test on synthetic data}
% %\vskip -0.2in
% \label{fig.scalability}
% \end{figure}

\subsection{Efficiency Evaluation}

\begin{figure*}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure[\LATT]{
\label{fig.exp3_1}
\includegraphics[width=0.205\linewidth]{./Figure/EXP3_LATT.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\LNUR]{
\label{fig.exp3_2}
\includegraphics[width=0.205\linewidth]{./Figure/EXP3_LNUR.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\ANIM]{
\label{fig.exp3_3}
\includegraphics[width=0.205\linewidth]{./Figure/EXP3_ANIM.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\IMAGE]{
\label{fig.exp3_4}
\includegraphics[width=0.205\linewidth]{./Figure/EXP3_IMAGE.eps} }\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[\YAGO]{
\label{fig.exp3_5}
\includegraphics[width=0.205\linewidth]{./Figure/EXP3_YAGO.eps} }%\hskip -0.15in
%\hspace{-0.29cm}
}
\vspace{-0.3cm}
\caption{Running time of different methods on all datasets.}% Here, $k=25$.}
\label{fig.exp3}
\vspace{-0.5cm}
\end{figure*}

\stitle{Exp-4: Efficiency evaluation.}
We evaluate the running time of four methods \greedy, \DP, \Baseline and \brute on all five datasets. \DP and \brute are optimal methods and \greedy and \Baseline are approximate methods. Figure~\ref{fig.exp3} shows running time of all methods when varying $k$. \greedy runs the fastest among them, which adopts an easy-to-compute greedy strategy. Interestingly, the efficiency of \DP is close to \greedy for small $k$ values. For the optimal methods, \DP is much faster than \brute. Note that the running time results of \greedy and \DP are similar and scale well on large-scale tree datasets \IMAGE and \YAGO, as we invoke the \vtree algorithm to reduce the tree size of  \IMAGE and \YAGO into a very small one in $O(|\mathcal{I}|)$.
% tree reduction in  because after , the size of \YAGO is similar with \IMAGE. %\revision{}
%We evaluate the running time of three methods \DP, \GVDO,  and \brute on trees. \DP and \brute are optimal methods and \GVDO is an approximate method.  Figure~\ref{fig.exp6} shows running time of all methods when varying $k$. \GVDO runs the fastest among them. Interestingly, the efficiency of \DP is close to \GVDO for small $k$ values.   For the optimal methods, DP is much faster than \brute. 

\begin{table}[t]
%\vspace{-0.2cm}
\centering
%\vspace{-0.3cm}
\caption{The size of new tree $T^*$ reduced by \vtree.}\label{table.exp4}
\vspace{-0.3cm}
\scalebox{1.0}{
\begin{tabular}{c|c|c|c|c|c}
\toprule
Datasets& LATT& LNUR& ANIM& IMAGE& YAGO \\
\midrule
$|T|$& 4,226& 4,226 & 15,135& 73,298& 493,839\\
$|\mathcal{I}|$& 960 & 771 & 4,350& 5,000& 10,000\\
$|T^*|$& 1,233 & 994 & 4,373& 6,402& 14,131\\
\bottomrule
\end{tabular}
}
%\vspace{-0.2cm}
%\caption{The results of $\g(S)$ on  tree datasets}\label{table.exp2}
%Summary score $\g(S)$ of \GVDO and \DP on  tree datasets}\label{table.exp2}
\vspace{-0.5cm}
\end{table}


\stitle{Exp-5: The size of reduced tree by Vtree.}
To verify the effectiveness of \vtree in Algorithm~\ref{algo:vtree}, we report the size of new trees $T^*$ reduced from $T$ on all real-world datasets. Table \ref{table.exp4} shows the size of original tree as $|T|$, the number of nodes with positive weights as $|I|$, and the size of new tree $|T^*|$ by \vtree. The size of new tree $|T^*|$ is much smaller than the original tree size $|T|$. $|T^*|$ is also smaller than two times of $|\mathcal{I}|$, which confirms the results of Theorem~\ref{theorem.treesize}.

\begin{figure}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure[Compute $\triangle_{g}(x|S)$(Seconds)]{
\label{fig.exp6_1}
\includegraphics[width=0.48\linewidth]{./Figure/EXP6_1.eps} }%\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[Running time(Seconds)]{
\label{fig.exp6_2}
\includegraphics[width=0.48\linewidth]{./Figure/EXP6_2.eps} }%\hskip -0.15in
%\hspace{-0.29cm}
}
\vspace{-0.3cm}
\caption{Scalability test on large synthetic datasets. Here, $k = 10$.}% Here, $k=25$.}
\label{fig.exp6}
\vspace{-0.4cm}
\end{figure}

\stitle{Exp-6 Scalability test.} In this experiment, we evaluate the scalability of \greedy and \DP by varying the size of tree $|\mathcal{V}|$. We randomly generate 5 trees with size varying from $10^5$ to $10^6$, whose  graph statistics follow the real dataset \LATT.  We set the parameter $k = 10$. 
First, we test the scalability of computing  $\triangle_{g}(x|S)$. Note that the operation of  $\triangle_{g}(x|S)$ is to compute the marginal gain of summary scores, which is only used in greedy algorithms but not the global optimal \DP method. Thus, we only compare two greedy methods \Baseline and \greedy here. The running time results of computing  $\triangle_{g}(x|S)$ by Baseline and \greedy are shown in Figure \ref{fig.exp6_1}.
%In addition, to verify the efficiency of computing  $\triangle_{g}(x|S)$ by the Algorithm \ref{algo:gain}, we compare approach \Baseline and \greedy. \revision{with greedy method}
%The results of running time are shown in Figure \ref{fig.exp6_1}. 
As we can see, \greedy is scalable very well with the increased size of tree nodes $|\mathcal{V}|$.
Moreover, \greedy is much more efficient than \Baseline, which verifies the efficiency of fast computing $\triangle_{g}(x|S)$ in Algorithm~\ref{algo:gain}. 
Next, we evaluate the scalability of top-$k$ tree summarization by \greedy and \DP. 
 Figure~\ref{fig.exp6_2} reports the running time results on the increased tree datasets. As expected,  \greedy and \DP take longer time with the increasing $|V|$ stably, indicating that both methods scale well with the increased $|\mathcal{V}|$.

\subsection{Case Study and Usability Evaluation}

\begin{figure}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure{
\includegraphics[width=0.95\linewidth]{./Figure/case_study.pdf} }%\hskip -0.15in
%\hspace{-0.29cm}
}
\vspace{-0.3cm}
\caption{A case study of tree summarization in ACM Computing Classification System (CCS). The vertex weight is the cumulative number of papers published under the corresponding topic. The topic that has more than 20,000 papers, is depicted in red bold.}
\label{fig.exp7}
\vspace{-0.4cm}
\end{figure}

\begin{figure}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure[OVDO]{
\label{fig.exp7_2_1}
\includegraphics[width=0.54\linewidth]{./Figure/case_study_1.pdf} }%\hskip -0.15in
%\hspace{-0.29cm}
\subfigure[GVDO]{
\label{fig.exp7_2_2}
\raisebox{0.3\height}{\includegraphics[width=0.42\linewidth]{./Figure/case_study_2.pdf}} }%\hskip -0.15in
%\hspace{-0.29cm}
}
\vspace{-0.3cm}
\caption{Graph visualization of top-$k$ summarization results by \greedy and \DP on ACM CCS dataset. Here, $k = 5$.}% Here, $k=25$.}
\label{fig.exp7_2}
\vspace{-0.4cm}
\end{figure}

\begin{figure}[t]
%\scriptsize
%\vspace{-0.5cm}
\centering
{
%\hspace{-1cm}
\subfigure{
\includegraphics[width=0.5\linewidth]{./Figure/user_study.pdf} }%\hskip -0.15in
%\hspace{-0.29cm}
}
\vspace{-0.3cm}
\caption{Usability evaluation of different methods for top-$k$ attractive topic recommendation on ACM CCS dataset in Figure~\ref{fig.exp7}.}
\label{fig.exp7_3}
\vspace{-0.4cm}
\end{figure}

In this experiment, we conduct case study and usability evaluation to validate the practical usefulness of our tree summarization model and algorithms. We construct a new real-world dataset with weighted terminologies from the ACM Computing Classification System (CCS)~\cite{}, as shown in Figure~\ref{fig.exp7}. The hierarchical tree has 17 vertices, where each vertex represents a topic. An edge between two topics represents that the parent vertex is a generalized concept of its children topics; A child vertex is an instance concept of its parent topic. For example, the ``computing methodology'' topic (denoted as T1) generalizes two subcategories of `Artificial Intelligence' (denoted as T4, `AI') and `Machine Learning' (denoted as T5, `ML'). Moreover, each vertex is associated with a weight, representing the cumulative number of papers published under its topic in ACM DL~\cite{} from 2011 to 2021. For example, there exist at least 61,000 published papers related to ``Computer Version'' topic (denoted as T12, 'CV'). 
The higher the vertex weight, the more attractive the topic.


\stitle{Exp-7: Case study of summary topics in graphical visualization.} We apply our summarization methods \greedy and \DP on the constructed ACM CCS dataset above. We set a small parameter $k=5$ to use only 5 topics to summarize the whole topic tree. 
%We compare the \greedy and \DP for $k = 5$ here. 
Figures~\ref{fig.exp7_2}(a) and~\ref{fig.exp7_2}(b) show the topic selections of \DP and \greedy, respectively. \DP selects five vertices T1, T2, T3, T5, and T12, which cover three general attractive topics ``computing methodology'', ``information system'', ``security \& privacy'', and two attractive topics ``ML'' and ``CV''. Note that we add a virtual root to connect with three vertices T1, T2, and T3, which follows the methodology of graphical visualization in Section~\ref{sec.visualization}. On the other hand, \greedy selects a different answer of five vertices T0, T5, T6, T7, and T12 as shown in Figure~\ref{fig.exp7_2}(b). This greedy method always first selects T0 no matter what kinds of parameter setting on $k$. The greedy summary result in Figure~\ref{fig.exp7_2}(b) has one obvious shortcoming that cannot cover the topic of security $\&$ privacy (denoted as T3). Thus, this greedy answer is worse than the optimal answer in Figure~\ref{fig.exp7_2}(a), which has a more diverse coverage of  different important topics and a larger summarization score.  

\stitle{Exp-8: Usability evaluation of summary topics.}  We conduct the usability evaluation for top-$k$ attractive topic recommendation, which selects $k$ topics to summarize attractive topics in ACM CCS dataset. We apply five methods \DP, \greedy, \AGG, \FEQ, and \TS on the constructed ACM CCS dataset. Note that \AGG and \CAGG select the same topics, thus only the topic selections of \AGG are reported here. We set $k=5$ and conduct a survey investigation.  Specifically, we ask 20 users, who are familiar with academic research and computer science topics. We request them to recommend top-5 most attractive topics of ACM CCS dataset in Figure~\ref{fig.exp7}. We evaluate an accuracy rate of matching topics between the users' choices and the methods' selections. Figure~\ref{fig.exp7_3} reports the average accuracy rate for all methods. Our method \DP achieves an accuracy rate of \revision{exact? more than 80\%}, which is the best performance among all methods. \greedy achieves \revision{exact? nearly 60\%} accuracy, while other methods achieve \revision{exact? less than 50\%}. This usability evaluation validate the usefulness of our methods in attractive topics summarization on ACM CCS dataset.


% \stitle{\revision{Exp-7. Case study and user study.}} 
% \revision{In this experiment, we conduct a case study of attractive topics summarization in ACM Computing Classification System. We built a hierarchical tree using 17 topics, as shown in Figure~\ref{fig.exp7}. The edges in the tree represent that parent topics can summarize its children topics. For example, ``computing methodology'' is the parent topic of ``AI'' and ``ML''. The weight of each node is the cumulative number of papers (from 2011 to 2021, collected from ACM DL) under the corresponding topic. The higher the number of papers, the more attractive the topic. We compare the \greedy and \DP for $k = 5$ here. Figure~\ref{fig.exp7_2} shows the selection of \DP and \greedy. \DP selects T1, T2, T3, T5, and T12, which cover three general attractive topics ``computing methodology'', ``information system'', ``security \& privacy'', and two attractive topics ``ML'' and ``CV''.  While, \greedy selects the vertex T0, T5, T6, T7, and T12 greedily because \greedy first selects T0 and it will be always in the selection. %For $k = 5$, \DP selects T1, T2, T3, T5, and T12, and \greedy selects T0, T5, T6, T7, and T12. \\
% }

%\revision{Except the case study, we also conduct a usability test of attractive topic recommendation for five methods \DP, \greedy, \AGG, \FEQ, and \TS. Note that \AGG and \CAGG select same topics, so we just report \AGG here. We ask 20 users, who are familiar with computer science topics, to recommend top-5 most attractive topics in ACM CCS (Figure~\ref{fig.exp7}). We evaluate an accuracy rate of overlapping topics between users' choices and methods' selections. Figure~\ref{fig.exp7_3} shows the average accuracy rate for all methods. Our method \DP achieves more than 80\% accuracy, which is the best. \greedy achieves nearly 60\% accuracy, while other methods achieve less than 50\%. This indicates an easy usability of our methods in attractive topics summarization of ACM CCS.}
